Exploring Grid Polygons Online

We investigate the exploration problem of a short-sighted mobile robot moving in an unknown cellular room. To explore a cell, the robot must enter it. Once inside, the robot knows which of the 4 adjacent cells exist and which are boundary edges. The robot starts from a specified cell adjacent to the room's outer wall; it visits each cell, and returns to the start. Our interest is in a short exploration tour; that is, in keeping the number of multiple cell visits small. For abitrary environments containing no obstacles we provide a strategy producing tours of length S <= C + 1/2 E - 3, and for environments containing obstacles we provide a strategy, that is bound by S <= C + 1/2 E + 3H + WCW - 2, where C denotes the number of cells-the area-, E denotes the number of boundary edges-the perimeter-, and H is the number of obstacles, and WCW is a measure for the sinuosity of the given environment.

==> SmartDFSCompTryI.tex <==
%----------------------------------------------------------------------
\iffalse
\begin{ass}{sdfscomp}
The strategy \smartDFS\ is competitive with a factor of
$\frac43$.
\end{ass}

\pstexfig{\smartDFS\ compared to the optimal strategy in a corridor of
width three.}{sdfscomp}

\begin{proof}(Idea)
Besides from experimental results, the conjecture is based upon the
following observation: Corridors of width one or two are explored
optimally by \smartDFS, so we achieves a factor of 1 in this cases.
In contrast, a rectangle of size $3\times m$ is explored with
$4m-2$ steps. The optimal strategy needs at least $3m$ steps, see
\reffig{sdfscomp}. This yields a factor of $\frac43$ for a large $m$.

\smallskip\noindent
Now, we observe possible modifications to the $3\times m$ rectangle.

\pstexfig{(i) Corridor of width $n>3$, (ii) Corridor with narrow passage.}
{sdfscomp2}

\begin{description}
\item[Broaden the corridor]~\\
We observe a corridor of size $n\times m$ with $3<n\leq m$. If $n$ is even,
the corridor is explored optimally, so let $n$ be odd.
\smartDFS\ needs $nm-1$ steps to visit every cell, $m-{n-1 \over 2}-1$ steps
for the horizontal part of the return path and ${n-1 \over 2}$ steps for
the vertical part, see \reffig{sdfscomp2}(i). This yields a factor of
$${mn+m-2\over mn} = 1+ \frac1n - {2\over mn} < \frac43 \mbox{ for } n>3.$$

\item[Add narrow passages]~\\
Adding a narrow passage causes a split cell and the narrow passage is
explored optimally, see \reffig{sdfscomp2}(ii). Therefore, the
competetive factor in this polygon is slightly smaller.

\item[Bend the corridor]~\\
Bending the corridor counterclockwise decreases the number of steps
by 2 for every bend.
Bending the corridor clockwise does not affect the number of steps, so
the competitive factor in a bended corridor is not worse than in a
straight corridor with the same number of cells.

\item[Add branches]~\\
%Branches of width one or even width are explored optimally, so the factor
%in a polygon with such a branch will be smaller than $\frac43$.
\REMARK{TODO}
\end{description}

\REMARK{Noch zu zeigen: mit diesen Transformationen lassen sich alle
Polygone generieren. Alternative: Induktion???}

\end{proof}
\fi
%----------------------------------------------------------------------
 
\bigskip
So far we have shown an upper bound for the number of steps needed
to explore a polygon that depends on the number of cells and
edges in the polygon. Now, we want to analyze \smartDFS\ 
in the competitive framework. We need two short lemmata to
give a competitive factor for \smartDFS.

\pstexfig{(i) Polygon of size $3\times m$. The number of cells in the
1-offset equals ${C(P)\over 3}-2$. (ii) In a corridor narrower than 3 the
1-offset gets disconnected.}
{sdfscomp2}

\begin{lem}{cellsthird}
Let $P$ be a simple grid polygon and $P'$ the 1-offset of $P$.
If $P'$ is connected, the shortest path between 
two cells in $P'$ is not longer than $\frac13\, C(P)-2$.
\end{lem}
\begin{proof}
Let $P$ be a corridor of width $3$.
$P'$, \ie\ the 1-offset of $P$, is a corridor of width 1, and a path 
in $P'$ is not longer than $C(P')-1 <C(P')$.
We can cut $P$ into ${C(P)\over 3}$ 'slices' of cells, see 
\reffig{sdfscomp2}(i).
The first and the last slice belong to the first layer of $P$. In
the remaining slices, 2 cells belong also to the first layer of $P$, just
one cell is left for the $P'$. Thus, $C(P')=\frac13\,C(P)-2$ holds.

It is easy to see, that if we have a wider corridor, the number of cells
in $P$ gets significally larger, while a shortest path in $P'$ 
increases at most one step for every additional layer.
If we narrow the corridor, the 1-offset gets disconnected, see
\reffig{sdfscomp2}(ii).
\end{proof}

\begin{lem}{excessthird}
Let $P$ be a simple grid polygon and $P'$ the 1-offset of $P$.
If $P'$ is connected, $\excess(P) \leq \frac13\, C(P)$ holds.
\end{lem}
\begin{proof}
$\excess(P)$ is the length of the shortest path from the last
explored cell, $t$, in $P$ back to the start cell, $s$. Since 
$P'$ is connected, we can circle the whole polygon in the first layer.
This path ends in a cell that touches $s$. After this we continue
with the second layer of $P$. Therefore, $t$ is located in $P'$. 
The shortest path from the start cell of $P'$, 
\ie\ the first cell in the second layer of $P$, is at most 2, 
because both cells touch each other, so
$\excess(P)\leq \excess(P')+2$ holds. With \reflem{cellsthird}
we get $\excess(P) \leq \frac13\, C(P)$.
\end{proof}

\pstexfig{In a corridor of width 3 $S(P)=\frac43\, \rmsub{S}{Opt}(P)$ holds.}
{sdfscomp}

\medskip\noindent
With \reflem{cellsthird} and \reflem{excessthird} we are able to proof
the following:

\begin{theo}{sdfscomp}
The strategy {\smartDFS} is competitive with a factor of
$\frac43$. This bound is tight.
\end{theo}
\begin{proof}
\smartDFS\ performs two types of operations: either it surrounds a 
layer of $P$ completely, because no split cell is detected in this layer,
or it handles a split cell. We will proof our statement by an induction
over the number of layers.

For the induction base consider a rectangle of size $n\times m$, 
$n\in\{1,2,3\}$.
For $n=1$ or $n=2$ the polygon is explored optimally. For $n=3$ 
we get with \reflem{excessthird} $\excess(P) \leq \frac13\, C(P)$
and thus 
$$S(P)=C(P)+\excess(P)\leq \frac43\, C(P)\leq \frac43\,\rmsub{S}{Opt}(P),$$
where $S(P)$ denotes the number of steps needed by \smartDFS\ and
$\rmsub{S}{Opt}(P)$ the length of the optimal path. Remark, that the
bound is tight if $m$ is even, see \reffig{sdfscomp}.

Now, we consider a simple polygon. Since dead ends of width one and two
are explored optimally, we can cut off these dead ends without changing the
competitive factor. Let $P$ be the resulting polygon.

If the first layer of $P$ contains no split cell, the competitive
factor follows as above from \reflem{excessthird}. Otherwise, let $c$ be the
first split cell in the first layer of $P$. As above, let $K_2$ be the
component that is visited first, $K_1$ be the other component. 
Two cases occur.

\pstexfig{Two cases occur if a split cell is found in the first layer.}
{sdfscomp2cases}

{\bf Case 1:} $K_2$ is not yet surrounded by the current layer 
(component of type (II)), see \reffig{sdfscomp2cases}(i).
Let 
$$P_1 := K_1 \cup \{\,\mbox{cells in the current layer that 
are already visited}\,\}$$ 
and let $P_2 := K_2 \cup \{c\}$. Note, that in this case
$P_1 \cap P_2 = \{c\}$ holds. Now, we can conclude
\begin{eqnarray*}
S(P) &=& S(P_1) + S(P_2)\\
&\leq& \frac43\,\rmsub{S}{Opt}(P_1) + \frac43\,\rmsub{S}{Opt}(P_2)
\quad\mbox{by induction hypothesis}\\
&\leq& \frac43\,\rmsub{S}{Opt}(P)
\end{eqnarray*}
The last inequation holds, because $P_1$ and $P_2$ overlap in only one
cell. The only thing the optimal strategy can do to explore $P$ is,
to explore the part of $P$ corresponding to $P_1$ up to $c$, continue
with the part of $P$ corresponding to $P_2$ and finish with the
rest of $P_1$. Therefore, the length of the optimal path in $P$ cannot
be shorter than $\rmsub{S}{Opt}(P_1) + \rmsub{S}{Opt}(P_2)$.

\smallskip
{\bf Case 2:} $K_2$ is completely surrounded by the current layer 
(component of type (I)).
This case occurs, because the robot meets a touching cell, $c'$, in the
same layer as $c$, see \reffig{sdfscomp2cases}(ii). 
Let $Q$ be the smallest rectangle that contains both $c$ and $c'$.
Choose $P_2$, such that $K_2$ is the 1-offset of $P_2$, and 
$P_1 := ( P\backslash P_2 ) \cup Q$.
Since $c$ and $c'$ are touching, $C(Q) \leq 4$  and thus
$C(P)\geq C(P_1)+C(P_2)-4$ holds. 
Analogously to \reflem{component} we have
$$\excess(P) = \excess(P_1) + \excess(K_2 \cup \{c\}) + 1\,.$$
Since $c$ and the start cell in $K_2$ are adjacent, 
$\excess(K_2 \cup \{c\}) = \excess(K_2) + 1$ holds, which yields
$$\excess(P) = \excess(P_1) + \excess(K_2) + 2.$$
Now, we apply the induction hypothesis to $P_1$ and \reflem{cellsthird}
to $K_2$ and get
\begin{eqnarray*}
\excess(P) &=& \frac13\,C(P_1) + \frac13\,C(P_2)\\
&\leq & \frac13\,C(P)-\frac43\\
&<& \frac13\,C(P)
\end{eqnarray*}
Thus, in every case $S(P)\leq \frac43\,\rmsub{S}{Opt}(P)$ holds.
\end{proof}


==> SmartDFSCompTryII.tex <==
 
\bigskip
%So far we have shown an upper bound for the number of steps needed
%to explore a polygon that depends on the number of cells and
%edges in the polygon. 
Now, we want to analyze \smartDFS\ 
in the competitive framework. We need two short lemmata to
give a competitive factor for \smartDFS.

\pstexfig{(i) Polygon of size $3\times m$. The number of cells in the
1-offset equals ${C(P)\over 3}-2$. (ii) In a corridor narrower than 3 the
1-offset gets disconnected.}
{sdfscomp2}

\pstexfig{(i) Polygon of size $3\times m$. The number of cells in the
1-offset equals ${C(P)\over 3}-2$, (ii) bending or (iii) adding
T-crossings does not change this.}{sdfscompslicesALT}

\begin{lem}{cellsthird}
Let $P$ be a simple grid polygon and $P'$ the 1-offset of $P$.
If $P'$ is connected, the shortest path between 
two cells in $P'$ is not longer than $\frac13\, C(P)-2$.
\end{lem}
\begin{proof}
Let $P$ be a corridor of width $3$.
$P'$, \ie\ the 1-offset of $P$, is a corridor of width 1, and a path 
in $P'$ is not longer than $C(P')-1 <C(P')$.
We can cut $P$ into ${C(P)\over 3}$ 'slices' of cells, see 
\reffig{sdfscomp2}(i).
The first and the last slice belong to the first layer of $P$. In
the remaining slices, 2 cells belong also to the first layer of $P$, just
one cell is left for the $P'$. Thus, $C(P')=\frac13\,C(P)-2$ holds.

It is easy to see, that if we have a wider corridor, the number of cells
in $P$ gets significally larger, while a shortest path in $P'$ 
increases at most one step for every additional layer.
If we narrow the corridor, the 1-offset gets disconnected, see
\reffig{sdfscomp2}(ii).
\end{proof}

\begin{lem}{excessthird}
For a simple grid polygon, $P$, without any dead ends of width one or two
and without any split cell, $\excess(P) \leq \frac13\, C(P)$ holds.
\end{lem}
\begin{proof}
Because we have no polygon split, $\excess(P)$ is the 
length of the shortest path from the last
explored cell, $t$, in $P$ back to the start cell, $s$, and
we can circle the whole polygon in the first layer.
This path through the first layer ends in a cell
$e$ that touches $s$, because $P$ has no dead ends of width one or two
that could cause the visit of the first layer to end anywhere else.

After the exploration of the first of $P$, we continue with the second
layer, starting from the first cell in the second layer, $s'$.
$s'$ touches both $s$ and $e$, and is adjacent to one of them. 
In both cases, on the path from $e$ to $s'$ and from $s'$ to $s$  
we visit two cells twice. Since we have to split cell and no 
narrow dead ends, $t$ is located in the 1-offset of $P$ and we have
$\excess(P)\leq \excess(P')+2$. With \reflem{cellsthird}
we get $\excess(P) \leq \frac13\, C(P) - 1$.
\end{proof}

\pstexfig{In a corridor of width 3 $S(P)=\frac43\, \rmsub{S}{Opt}(P)$ holds.}
{sdfscomp}

\medskip\noindent
With \reflem{cellsthird} and \reflem{excessthird} we are able to proof
the following:

\begin{theo}{sdfscomp}
The strategy {\smartDFS} is competitive with a factor of
$\frac43$. This bound is tight.
\end{theo}
\begin{proof}
\smartDFS\ performs two types of operations: either it surrounds a 
layer of $P$ completely, because no split cell is detected in this layer,
or it handles a split cell. We will proof our statement by an induction
over these operations, \ie\ over the number layers and polygon splits.

We consider a simple polygon. Since dead ends of width one and two
are explored optimally, we can cut off these dead ends without changing the
competitive factor. Let $P$ be the resulting polygon.

\hrulefill
For the induction base consider a rectangle of size $n\times m$, 
$n\in\{1,2,3\}$.
For $n=1$ or $n=2$ the polygon is explored optimally. For $n=3$ 
we get with \reflem{excessthird} $\excess(P) \leq \frac13\, C(P)$
and thus 
$$S(P)=C(P)+\excess(P)\leq \frac43\, C(P)\leq \frac43\,\rmsub{S}{Opt}(P),$$
where $S(P)$ denotes the number of steps needed by \smartDFS\ and
$\rmsub{S}{Opt}(P)$ the length of the optimal path. Remark, that the
bound is tight if $m$ is even, see \reffig{sdfscomp}.
\hrulefill

\pstexfig{Either $s'$ and $s$ or $s'$ and $e$ are ajacent. 
In both cases two cells in $P$ are visited twice (bold arrows).}
{sdfscompsprime}

{\bf Case 1:} The first layer of $P$ contains no split cell.
Thus, we can circle the whole polygon in the first layer.
The path through the first layer ends in a cell
$e$ that touches $s$, because $P$ has no dead ends of width one or two
that could cause the exploration of the first layer to end anywhere else.

After the exploration of the first of $P$, we continue with the second
layer, starting from the first cell in the second layer, $s'$.
$s'$ touches both $s$ and $e$, and is adjacent to one of them. 
In both cases, we visit two cells twice
on the path from $e$ to $s'$ and from $s'$ to $s$,
see \reffig{sdfscompsprime}.




 the competitive
factor follows as above from \reflem{excessthird}. Otherwise, let $c$ be the
first split cell in the first layer of $P$. As above, let $K_2$ be the
component that is visited first, $K_1$ be the other component. 
Two cases occur.

\pstexfig{Two cases occur if a split cell is found in the first layer.}
{sdfscomp2cases}

{\bf Case 1:} $K_2$ is not yet surrounded by the current layer 
(component of type (II)), see \reffig{sdfscomp2cases}(i).
Let 
$$P_1 := K_1 \cup \{\,\mbox{cells in the current layer that 
are already visited}\,\}$$ 
and let $P_2 := K_2 \cup \{c\}$. Note, that in this case
$P_1 \cap P_2 = \{c\}$ holds. Now, we can conclude
\begin{eqnarray*}
S(P) &=& S(P_1) + S(P_2)\\
&\leq& \frac43\,\rmsub{S}{Opt}(P_1) + \frac43\,\rmsub{S}{Opt}(P_2)
\quad\mbox{by induction hypothesis}\\
&\leq& \frac43\,\rmsub{S}{Opt}(P)
\end{eqnarray*}
The last inequation holds, because $P_1$ and $P_2$ overlap in only one
cell. The only thing the optimal strategy can do to explore $P$ is,
to explore the part of $P$ corresponding to $P_1$ up to $c$, continue
with the part of $P$ corresponding to $P_2$ and finish with the
rest of $P_1$. Therefore, the length of the optimal path in $P$ cannot
be shorter than $\rmsub{S}{Opt}(P_1) + \rmsub{S}{Opt}(P_2)$.

\smallskip
{\bf Case 2:} $K_2$ is completely surrounded by the current layer 
(component of type (I)).
This case occurs, because the robot meets a touching cell, $c'$, in the
same layer as $c$, see \reffig{sdfscomp2cases}(ii). 
Let $Q$ be the smallest rectangle that contains both $c$ and $c'$.
Choose $P_2$, such that $K_2$ is the 1-offset of $P_2$, and 
$P_1 := ( P\backslash P_2 ) \cup Q$.
Since $c$ and $c'$ are touching, $C(Q) \leq 4$  and thus
$C(P)\geq C(P_1)+C(P_2)-4$ holds. 
Analogously to \reflem{component} we have
$$\excess(P) = \excess(P_1) + \excess(K_2 \cup \{c\}) + 1\,.$$
Since $c$ and the start cell in $K_2$ are adjacent, 
$\excess(K_2 \cup \{c\}) = \excess(K_2) + 1$ holds, which yields
$$\excess(P) = \excess(P_1) + \excess(K_2) + 2.$$
Now, we apply the induction hypothesis to $P_1$ and \reflem{cellsthird}
to $K_2$ and get
\begin{eqnarray*}
\excess(P) &=& \frac13\,C(P_1) + \frac13\,C(P_2)\\
&\leq & \frac13\,C(P)-\frac43\\
&<& \frac13\,C(P)
\end{eqnarray*}
Thus, in every case $S(P)\leq \frac43\,\rmsub{S}{Opt}(P)$ holds.
\end{proof}


==> figCells/3dmodell_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(9044,3248)(-471,-5087)
\put(5446,-5011){\makebox(0,0)[b]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(ii)}%
}}}}
\put(451,-5011){\makebox(0,0)[b]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(i)}%
}}}}
\end{picture}%


==> figCells/AlwaysReserveFails_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5016,1866)(1318,-2794)
\put(2926,-2626){\makebox(0,0)[b]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\itdefault}{\color[rgb]{0,0,0}\( s \)}%
}}}}
\end{picture}%


==> figCells/CellExplSPNoBenefit_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(7266,6366)(1768,-5944)
\end{picture}%


==> figCells/CellExplSPTight2_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5016,4566)(3118,-5494)
\end{picture}%


==> figCells/CellExplSPTightALT_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5916,3666)(3118,-4144)
\end{picture}%


==> figCells/CellExplSPTight_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5466,4566)(3118,-5494)
\end{picture}%


==> figCells/CellExplTight_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3216,2766)(3568,-4594)
\end{picture}%


==> figCells/CellPoly_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6795,2269)(1768,-3647)
\put(7876,-3571){\makebox(0,0)[b]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(ii)}%
}}}}
\put(3376,-3571){\makebox(0,0)[b]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(i)}%
}}}}
\end{picture}%


==> figCells/ComplexExample_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(9538,7738)(4007,-7305)
\end{picture}%


==> figCells/NoFwdSteps_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5874,2949)(664,-2548)
\end{picture}%


==> figCells/ObstacleLayer1_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(7087,5038)(6257,-7755)
\end{picture}%


==> figCells/ObstacleLayer1_mail_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(7361,5038)(6257,-7755)
\end{picture}%


==> figCells/PumpingProblem_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5016,6388)(5829,-7755)
\end{picture}%


==> figCells/SPBenefit_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(11274,3553)(664,-6077)
\put(3376,-6001){\makebox(0,0)[b]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(i)}%
}}}}
\put(9226,-6001){\makebox(0,0)[b]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(ii)}%
}}}}
\end{picture}%


==> figCells/ThreeComponentsProblem_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6838,6388)(4007,-7755)
\put(10711,-5686){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\itdefault}{\color[rgb]{0,0,0}\( s \)}%
}}}}
\end{picture}%


==> figCells/ThreeComponents_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(6838,6388)(4007,-7755)
\put(10711,-5686){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\itdefault}{\color[rgb]{0,0,0}\( s \)}%
}}}}
\end{picture}%


==> figCells/XYmonotone_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5488,2788)(1517,-5295)
\put(1951,-3166){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\itdefault}\( \Pi \)}}}}
\end{picture}%


==> figCells/assumption_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2481,1329)(1564,-3403)
\put(3061,-2536){\makebox(0,0)[lb]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}blocked}%
}}}}
\end{picture}%


==> figCells/fwdsteps_1.tex <==
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(12060,20274)(-410,-20323)
\end{picture}%


==> figCells/ltsteps1_1.tex <==
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(13749,14874)(664,-14923)
\end{picture}%


==> figCells/ltsteps2_1.tex <==
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(13749,14874)(664,-14923)
\end{picture}%


==> figCells/ltsteps3_1.tex <==
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(13974,14874)(1789,-14923)
\end{picture}%


==> figCells/ltsteps4_1.tex <==
\setlength{\unitlength}{1657sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(14019,16674)(1744,-16723)
\end{picture}%


==> figCells/oddcorridor_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(9966,3643)(1318,-5492)
\put(3466,-5416){\makebox(0,0)[lb]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(i)}%
}}}}
\put(9271,-5416){\makebox(0,0)[lb]{\smash{{\SetFigFont{10}{12.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(ii)}%
}}}}
\end{picture}%


==> figCells/sdfslowerbound2_1.tex <==
\setlength{\unitlength}{2072sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2519,2069)(4029,-4808)
\end{picture}%


==> problems.tex <==
\clearpage
\sect{Solved and unsolved problems}{probl}

\pstexfig{Two Components, $d=3$, square width $=2d+1$.}{TwoComponents}

\pstexfig{Two Components, $d=3$ in $P_2$, square width $=2d$.}{TwoComponentsAsym}

\pstexfig{Two Components, similar to \reffig{TwoComponentsAsym}.}{TwoComponentsAsym2}

\pstexfig{Two Components, also similar to \reffig{TwoComponentsAsym}?}{TwoComponentsAsym3}

\pstexfig{Three Components, $d=3$, square width $=2d+1$.}{ThreeComponents}

\pstexfig{Three Components, $d=??$, square??}{ThreeComponentsProblem}

